Community detection with node attributes in multilayer networks

Community detection in networks is commonly performed using information about interactions between nodes. Recent advances have been made to incorporate multiple types of interactions, thus generalizing standard methods to multilayer networks. Often though, one can access additional information regarding individual nodes, attributes or covariates. A relevant question is thus how to properly incorporate this extra information in such frameworks. Here we develop a method that incorporates both the topology of interactions and node attributes to extract communities in multilayer networks. We propose a principled probabilistic method that does not assume any a priori correlation structure between attributes and communities but rather infers this from data. This leads to an efficient algorithmic implementation that exploits the sparsity of the dataset and can be used to perform several inference tasks; we provide an open-source implementation of the code online. We demonstrate our method on both synthetic and real-world data and compare performance with methods that do not use any attribute information. We find that including node information helps in predicting missing links or attributes. It also leads to more interpretable community structures and allows the quantification of the impact of the node attributes given in input.

==> Sections/A_case_study.tex <==
% !TEX program = pdflatex
% !TEX root = ../mtcov.tex

\chapter{A Case Study}
\label{sec: A Case Study}
\thispagestyle{empty}

In this chapter, we present some applications to real-networks, in order to demonstrate the strengths of our model. We show improvements in terms of the evaluation measures compared to the version of the algorithm that does not consider the attributes, and highlight the interpretability of the results. In section \ref{data}, we start by describing the network data and summarizing their descriptive characteristics. Then, we present the analysis, the main issues and the results. In the last section of this chapter, we provide both quantitative and qualitative conclusions.

\section{Data}
\label{data}
We analyzed three real-networks that describe the social support interactions between residents of two South Indian villages, that are named by pseudonyms `Te\underline{n}pa\d{t}\d{t}i' (TEN) and `A\underline{l}ak\={a}puram' (ALA), for privacy reasons. The data have been collected by the anthropologist E. A. Power with help from Madurai Kamaraj University and Chella Meenakshi Centre for Education Research and Services, into two rounds: one in 2013 and the other in 2017.  The surveys have been approved by Human Subjects Institutional Review Board of Stanford University and of the University of Cincinnati, respectively. More details about datasets and background of the data research can be found in \shortciteA{E.A.Power.dissertation} and \shortciteA{E.A.Power.Nature}.
The social support surveys were conducted with virtually all adult residents of the two villages and they were asked to name those individuals who are their close friends or relatives, who provided them with different types of support (e.g. money loan, advice) and who plays a particular role within the village. Each question about social support and reputation endorsement has been translated in a layer in the respective network. In addition, some metadata were collected, which include features like age, religion, caste, education and so on.\\

\noindent In previous works, \shortciteA{E.A.Power.dissertation} and \shortciteA{E.A.Power.Nature} considered the hypothesis that there is a relationship between religion and prosociality, as well as \shortciteA{Multitensor} suggested an interdependence between the attribute caste and the mechanisms driving edge formation, which means the community structure. We based our analysis on the last hypothesis, assuming an underlying dependence between the communities, the multilayer structure and the compositional dimension given by the attribute caste. Raw data have been pre-processed first. We kept only residents and survey respondents who had at least one edge among the layers. Moreover, we considered the networks without self-loops. Then, the resulting directed networks present the characteristics showed in the Table \ref{tab: Statistics}, and we refer to them as TEN 2013, TEN 2017 and ALA 2017, respectively.
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cccccc}
\hline
\textbf{Village} & \textbf{Year} & \textbf{Nodes} & \textbf{Layers} & \textbf{Average Edges} & \textbf{Average Density} \\ \hline
Te\underline{n}pa\d{t}\d{t}i               & 2013          & 362            & 12              & 504.42                 & 0.386                    \\
Te\underline{n}pa\d{t}\d{t}i                & 2017          & 346            & 11              & 514.82                 & 0.431                    \\
A\underline{l}ak\={a}puram                & 2017          & 441            & 11              & 792.64                 & 0.408                    \\ \hline
\end{tabular}
\caption{Network summary statistics for the three adult resident village networks.}
\label{tab: Statistics}
\end{table}

\noindent The distribution of the attribute caste inside each network is shown in Figure \ref{fig: caste}. It displays some differences between `Te\underline{n}pa\d{t}\d{t}i' and `A\underline{l}ak\={a}puram' networks, but also a common unbalanced partition of the categories. This covariate is present with 10 categories in TEN 2013, 9 in TEN 2017 and 13 in ALA 2017.

\begin{figure}[!hp]

\centering
\begin{minipage}[b]{\textwidth}
\centering
\subfloat{\includegraphics[width=.7\linewidth]{./Figures/Caste_distr_ten13.png}}
\caption*{(a) TEN 2013.}
\subfloat{\includegraphics[width=.7\linewidth]{./Figures/Caste_distr_ten17.png}}
\caption*{(b) TEN 2017.}
\end{minipage}

\bigskip
\begin{minipage}[b]{\textwidth}
\centering
\subfloat{\includegraphics[width=.7\linewidth]{./Figures/Caste_distr_ala17.png}}
\caption*{(c) ALA 2017.}
\end{minipage}

\caption{Distribution of the attribute caste inside each network.}
\label{fig: caste}
\end{figure}


\section{Analysis}
In order to find the communities and measure their interdependence with the covariate, we analyzed the three networks  using the \textit{MTCov}  model already presented in chapter \ref{sec: The Model} and implemented in Python and R.
We started by investigating the behaviour of the global log-likelihood $\mathcal{L}$, as well as the two parts of which it is composed. Figure \ref{fig: log_normalization} shows an example for the network ALA 2017 and the attribute caste. The different scaling between $\mathcal{L_X}$ and $\mathcal{L_G}$ graphs is notable, which results in a different contribution on the final log-likelihood. For this reason, we first looked for a normalization procedure, in order to give a reasonable interpretation for the estimated scaling parameter $\hat{\gamma}$.

\begin{figure}[!ht]
             \centering
             \includegraphics[width=1.05\textwidth,height=\textheight,keepaspectratio]{./Figures/log_normalization.png}
\caption{Behaviours of the log-likelihood $\mathcal{L_X}$ (compositional dimension), the log-likelihood $\mathcal{L_G}$ (structural dimension) and the global log-likelihood $\mathcal{L}$. Here, we report results for the ALA 2017 network and the attribute caste, using $\gamma=0.6.$}
\label{fig: log_normalization}
\end{figure}

\subsection{Normalization}
Since the preliminary analysis highlighted a relation between the log-likelihoods, network structures and attributes, we estimated two linear regression models in order to obtain the normalization constants for the two sources of information. We collected log-likelihood values with respect to the number of nodes ($N$), edges ($E$) of the observed network and the number of categories of the categorical attribute ($Z$). Quantitatively, this means normalizing as:
\begin{align}
\label{normalization_eq}
    \mathcal{L} = \gamma \frac{\mathcal{L_X}}{c^\mathcal{X}_N N+c^\mathcal{X}_E E+c^\mathcal{X}_Z Z} + (1-\gamma)\frac{\mathcal{L_G}}{c^\mathcal{G}_N N+c^\mathcal{G}_E E+c^\mathcal{G}_Z Z}.
\end{align}
The super and the subscripts of the $c$ parameters indicate the dependent variable ($\mathcal{L_X}$ or $ \mathcal{L_G}$) and the input regressor they refer to, respectively. In particular, we collected the data by running the model for each pair of network and categorical attribute, arbitrarily fixing the number of communities $C=3$ and the scaling parameter $\gamma=0.5$. 
Table \ref{tab: Estimation} states the values of the coefficients which resulted statistically significant for the estimation of the log-likelihood terms\footnote{Only the statistically significant coefficients have been used in the normalized eq. (\ref{normalization_eq}).}.
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{ccc}
\hline
\textbf{} & \textbf{$\mathcal{L_X}$} & \textbf{$\mathcal{L_G}$} \\ \hline
$c_N$         & $-0.486^{***} $     & $-1.778^{**} $     \\
$c_E$         &             & $-6.158^{***}  $    \\
$c_Z$         & $-33.862^{***}$    &             \\ \hline
\end{tabular}
\caption{Coefficient estimates $c^\mathcal{X}_N$, $c^\mathcal{X}_E$, $c^\mathcal{X}_Z$, $c^\mathcal{G}_N$, $c^\mathcal{G}_E$ and $c^\mathcal{G}_Z$ for the two linear regression models.}
\label{tab: Estimation}
\end{table}

\noindent On one side, this procedure presented coefficient estimates useful for analyzing all three networks as automatically as possible, used in the algorithm for normalizing the respective log-likelihood terms before joining them. On the other side, we are aware that these coefficients are strictly related to the type of network we are working with. In this sense, future works should investigate an automatic normalization procedure for any network.

\subsection{Evaluation measures}
\label{em}
Given that we are considering attributed networks without ground-truth about community assignments, model evaluation is inherently challenging. Moreover, in this case we have an additional aspect to consider: the co-existence of multiple objective functions. In fact, we want to identify sets of nodes making a good cluster with respect to all these aspects \shortcite{bothorel2015clustering}. For this reason, we decided to define two different evaluation measures, one for the structure and the other for the attribute.\\

\noindent Even though there have been many recent developments in the literature about methods for evaluating graph clustering algorithms that rely on network structure, this is still an open problem as there is no general agreement about what are the best practices. For more details about existing methods, we refer the reader to the following works: \shortciteA{fortunato2010community}, \shortciteA{leskovec2010empirical}, \shortciteA{bothorel2015clustering} and \shortciteA{chakraborty2017metrics}.\\
Here, given the similarity of applications and contexts, we follow the approach used by \shortciteA{clauset2008hierarchical}. In particular, we developed a generative algorithm that allows the use of a link-prediction technique both for performing a hyperparameter tuning and for quantifying the accuracy of the predicted partitions. More specifically, we used the AUC statistic, equivalent to the area under the receiver-operating characteristic (ROC) curve \shortcite{hanley1982meaning}. It represents the probability that a randomly chosen missing connection (a true positive) is given a higher score by our method than a randomly chosen pair of unconnected vertices (a true negative). Thus, an AUC statistic equal to $0.5$ indicates random chance, while the closer it is to $1$, the more our model's predictions are better. A strong positive correlation between the community division and the link prediction has been confirmed also by \shortciteA{wu2018usi}.\\

\noindent For the attribute, instead, we used the accuracy as a quality measure. For each node, we computed the multinomial parameter $\pi_i$ using eq. (\ref{eq: piz}), given the estimated parameters $\hat{\beta}$ and the estimated community membership matrices $\hat{U}$ and $\hat{V}$. We then assigned to each node the category with the highest probability, computing the accuracy as a fraction between the corrected classified examples and the total number of nodes. We compared this value both with the random probability and the highest relative frequency in the training set.

\subsection{Hyperparameter tuning}
\label{ht}
In order to evaluate our model on the data, we designed a procedure for tuning the hyperparameters, which are defined as parameters that cannot be directly learned from the data, but usually fixed before the actual training process begins. Here, they are represented by the scaling parameter $\gamma$ and the number of communities $C$, given the unsupervised context. 
The optimal values are those who present the best performance of the model, and they have been chosen by using the $5$-fold Cross Validation technique in conjunction with the Grid Search strategy. Such approach consists in first splitting the dataset into $K$ folds: $K-1$ of them make the training set, the remaining fold is the test set (or held-out set). Secondly, repeatedly training the model from scratch on the $K-1$ folds of the sample and testing on the held-out fold, and this procedure is done for all combinations of the enumerated hyperparameters. Then, we choose the combination ($\hat{C},\hat{\gamma}$) that returns the best averaged performance over the cross-validation runs.
Although this procedure might be computationally expensive, it gives us the possibility to adapt our choice in order to have a co-existence of good performance for both objective functions. In fact, working with other strategies or optimization procedures would have returned the optimal value but these may not allow to compare \textit{jointly} the two values.\\

\noindent We choose, as range of possible values for $C$, the integer numbers in $[2, 15]$. In order to avoid a large number of groups, values greater than $15$ have not been considered, while the option $1$ corresponds to the trivial case without communities. For $\gamma$, we considered values in $[0,1]$, at intervals of equal length of $0.1$. Moreover, the dataset has been split as follows:
\begin{itemize}
    \item For the structure, instead of removing $20\%$ of the nodes or $20\%$ of the links, we hided $20\%$ of the entries of the adjacency matrix, including both zeros and ones, strategy used by \shortciteA{Multitensor}.
    \item For the attribute, we hided $20\%$ of the entries of the categorical vector.
\end{itemize}
In each iteration, we first trained the model giving as input the adjacency and the design matrices with hidden entries, then we tested on the elements of the fold left out. At each step, we computed both AUC and accuracy on the test set. Figure \ref{fig: TEN2013_K-cv} illustrates the average results for all combinations of the hyperparameters ($C, \gamma$), for the network TEN 2013. The plots of the other networks are attached in Appendix \ref{AA}. The blue and orange horizontal dashed lines represent the best cross-validation values for the two evaluation measures independently, while the black line displays the pair of selected hyperparameters. We chose as best parameters the pair that returns the closest values to the best for both objective functions. \\
\begin{figure}[!ht]
             \centering
             \includegraphics[width=1.0\textwidth,height=\textheight,keepaspectratio]{./Figures/5-cv_mean_TEN13_2.png}
\caption{$5$-fold CV average values for AUC and accuracy for all combinations of the hyperparameters for the network based on Te\underline{n}pa\d{t}\d{t}i village in the year 2013 and the attribute caste. The blue and orange dashed lines represent the best cross-validation values for the two evaluation measures independently, while the black one displays the pair of selected hyperparameters.}
\label{fig: TEN2013_K-cv}
\end{figure}



\noindent In order to assess if the presence of the covariate helps the algorithm for detecting communities, there are two straightforward models for comparison. One is given by the restricted \textit{MTCov}  model with scaling parameter $\gamma=0$, that allows to take into account only the structural dimension. The other model is represented by \textit{MultiTensor}, which only takes as input the adjacency tensor. However, before starting the validation phase, also the hyperparameter $C$ of these models needed to be set. We used the same $5$-fold CV technique, obtaining equivalent final choices for all networks with both models, as showed in Figure \ref{fig: cv_mt}. This was an expected result since the log-likelihood of the \textit{MultiTensorCov} model with $\gamma=0$ is only composed by the component $\mathcal{L_G}$, which is exactly the objective function of the \textit{MultiTensor} model. Moreover, the parameters updates for the two algorithms are almost the same, up to the normalization constants given by the fact that \textit{MTCov}  put some normalization restrictions, while \textit{MT} works in an unconstrained space.\\
\begin{figure}[!hp]
\centering
\includegraphics[scale=.4]{./Figures/5-cv_TEN13_mt.png}\\[.5\baselineskip]
\centering
\includegraphics[scale=.4]{./Figures/5-cv_TEN17_mt.png}\\[.5\baselineskip]
\centering
\includegraphics[scale=.4]{./Figures/5-cv_ALA17_mt.png}
\caption{$5$-fold CV average values for the AUC for all possible choices of the hyperparameter $C$, considering \textit{MT} and the restricted \textit{MTCov}  with $\gamma=0$.}
\label{fig: cv_mt}
\end{figure}

\noindent Table \ref{tab: tuning} summarizes the results of the hyperparameter tuning for the three algorithms, and these values are going to be used in the next section for validating the model. It should be noticed that \textit{MTCov}  estimated fewer communities, or at most the same number, than the comparison models. This is due to the presence of the scaling parameter $\gamma$, that captures the complexity of the data and helps during the formation of communities providing more information. In addition, this parameter ranges between $0.4$ and $0.6$, meaning that the two sources of information contribute almost equally for detecting the communities. Also, these values show a correlation between the structure, the attribute and the communities.

\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{ccccc}
\hline
                  &                                                      & \textbf{MT}                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Restricted\\ MTCov\end{tabular}} & \textbf{MTCov}                                   \\ \hline
\textbf{TEN 2013} & \begin{tabular}[c]{@{}c@{}}$\hat{C}$\\ $\hat{\gamma}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}12\\ ---\end{tabular} & \begin{tabular}[c]{@{}c@{}}12\\ 0\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}10\\ 0.4\end{tabular} \\ \hline
\textbf{TEN 2017} & \begin{tabular}[c]{@{}c@{}}$\hat{C}$\\ $\hat{\gamma}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}6\\ ---\end{tabular}  & \begin{tabular}[c]{@{}c@{}}6\\ 0\end{tabular}                       & \begin{tabular}[c]{@{}c@{}}6\\ 0.5\end{tabular}  \\ \hline
\textbf{ALA 2017} & \begin{tabular}[c]{@{}c@{}}$\hat{C}$\\ $\hat{\gamma}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}10\\ ---\end{tabular} & \begin{tabular}[c]{@{}c@{}}10\\ 0\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}9\\ 0.6\end{tabular}  \\ \hline
\end{tabular}
\caption{Values of the hyperparameters after tuning, for the three models and networks.}
\label{tab: tuning}
\end{table}

\section{Results}
\noindent Once the hyperparameters have been fixed, we assessed the performance of the model by validating its results both in terms of evaluation measures and interpretability of the communities. We analyzed the used networks considering the attribute caste, transformed by one hot encoding technique. Subsection \ref{val} describes the validation phase and the comparisons with the \textit{MultiTensor} and the restricted \textit{MultiTensorCov} models. Finally, in the subsection \ref{int} we show the detected communities and present their qualitative interpretations.

\subsection{Validation}
\label{val}
We quantitatively validated the model by performing ten independent runs with different training and test sets, for each network. In each experiment, the datasets have been split as explained in subsection \ref{ht}, using the $70\%$ for the training set and the $30\%$ for testing, and we adopted the evaluation measures previously introduced in subsection \ref{em}. For each trial, we estimated the $\Theta$ parameters on the training set, used in a second step for computing the AUC and the accuracy on the test set. For comparison, we run the \textit{MultiTensor} algorithm and the restricted version of our model, that considers only the structural part by fixing the scaling parameter $\gamma=0$. Moreover, we looked at other two baselines for the accuracy, such as the random probability assigned to each category of the attribute (RP) and the maximum relative frequency of the covariate caste in the training set (MRF).\\

\noindent Table \ref{tab: res1} shows the average results over ten runs for the considered networks, together with their standard deviations. In all cases, our algorithm achieves the highest accuracy for the caste category prediction, and in two cases over three the highest AUC for the edge prediction, indicated in boldface. Nonetheless, even in the single case where our model is not the best, the difference in score is negligible and can be offset by the possibility of inferring the attribute, feature that is distinctive of our method.

\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline  &  & \multicolumn{2}{c}{\textbf{TEN 2013}}  & \multicolumn{2}{c}{\textbf{TEN 2017}} & \multicolumn{2}{c}{\textbf{ALA 2017}} \\ \hline
\multirow{7}*{\textbf{\begin{tabular}[c]{@{}c@{}}ACCURACY\\ for the\\ covariate\\ caste\\ on the\\ test sets\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}RP\end{tabular} & & 0.1 & & 0.11  & & 0.08
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}MRF\end{tabular} &  & 0.318 $\pm$  0.014  & & 0.327 $\pm$  0.016  &  & 0.555 $\pm$  0.009
\\ \cline{2-8}
& MT  & $C = 12$  & ---  & $C = 6$  & ---  & $C = 10$ & ---  
\\ \cline{2-8} 
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.317 $\pm$  0.037
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & 0.381 $\pm$  0.028
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.597 $\pm$  0.028
\\ \cline{2-8} 
& MTCov
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & \textbf{0.342 $\pm$  0.050}
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & \textbf{0.407 $\pm$  0.033}
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.611 $\pm$  0.030} \\ \hline
\multirow{5}*{\textbf{\begin{tabular}[c]{@{}c@{}}AUC for the\\ link prediction\\ on the\\ test sets\end{tabular}}}
& MT  & $C = 12$  & \textbf{0.830 $\pm$  0.004} & $C = 6$  & 0.819 $\pm$  0.008  & $C = 10$ & 0.849 $\pm$  0.005 \\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.809 $\pm$  0.010
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & 0.832 $\pm$  0.002
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.867 $\pm$  0.006
\\ \cline{2-8}
& MTCov 
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & 0.825 $\pm$  0.012
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & \textbf{0.840 $\pm$  0.005} 
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.886 $\pm$  0.005}
\\\hline
\end{tabular}}
\caption{Performance of methods \textit{MT} , restricted \textit{MTCov}  and \textit{MTCov}  on three social networks. RP is the random probability baseline for the accuracy of the category of caste attribute prediction. MRF indicates the maximum relative frequency linked to the covariate caste in the training set. The results are averaged over ten independent runs and the best outcomes are bolded.}
\label{tab: res1}
\end{table}

\noindent To emphasize the importance of the covariate in the community detection task, we implemented experiments with non-random test and training sets. We used sampling bias techniques for assigning higher or lower sampling probability to the entries of the adjacency tensor, which correspond to edges than the non-edges ones. In particular, we assigned to the entries $a_{ij}^{\alpha}=1$ the probability given by 
\begin{align}
    p_1 = \frac{\text{total probability of picking up one edge (tpe)}}{\text{number of edges in the network (E)}} \ \ ,
\end{align}
and for $0$ entries
\begin{align}
    p_2 =\frac{1-\text{total probability of picking up one edge (tpe)}}{N - E} \ \ ,
\end{align}
where $N$ is the number of the nodes of the network.
The tpe was used to select entries for the test set; in case of selecting entries uniformly at random, this value would be around $0.003$. This low value is due to the common case in real networks of having sparse matrices, where the number of $1$ is much lower than the number of $0$. The aim was to assess the importance of having another source of information in situations where the number of positive examples in the training sets is not equally likely as the negative ones.\\
We created three different situations: 
\begin{itemize}
\item tpe $=0.002$: the probability of selecting one edge is lower than the probability of choosing one non edge, and the number of edges in the training set is much higher than the number in the test set.
\item tpe $=0.01$: the probability of selecting one edge is higher than the probability of choosing one non edge, and the number of edges in the training set is a bit smaller than the number in the test set.
\item tpe $=0.015$: the probability of selecting one edge in the test set is higher than the probability of choosing one non edge, and the test set has a bigger number of positive examples.
\end{itemize}
The presented frameworks follow an increasing order of complexity, starting from an over-represented case, where tpe $=0.002$, and ending with a difficult task where the number of edges in the training set is under-represented, tpe $=0.015$. We run 10 independent trials for each setting and model. The performances are shown in Figure \ref{fig: ev_biased}, where the opacity controls the complexity of the frameworks: the lower the value of tpe (less complex), the more transparent the opacity. Moreover, Tables \ref{tab: res2}, \ref{tab: res3} and \ref{tab: res4} present the results averaged over the independent runs, obtained in the three settings, respectively. 

\begin{figure}[!ht]
\centering
\includegraphics[width=0.75\textwidth]{./Figures/Evaluations_biased.png}
\caption{Probabilistic link prediction accuracy AUC of \textit{MTCov}  and \textit{MT}. The values of AUC for \textit{MTCov}  and \textit{MT} are shown on the vertical axis and the horizontal axis respectively. The opacity controls the complexity of the frameworks: on the left tpe $=0.015$ (high opacity and complexity), on the center tpe $=0.01$ (medium opacity), on the right tpe $=0.002$ (low opacity). Points above the diagonal,
shown in orange, are trials where \textit{MTCov}  is more accurate
than \textit{MT}. The fractions for which each method is superior
are shown in the plot legend.}
\label{fig: ev_biased}
\end{figure}

\begin{table}[htp]
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline  &  & \multicolumn{2}{c}{\textbf{TEN 2013}}  & \multicolumn{2}{c}{\textbf{TEN 2017}} & \multicolumn{2}{c}{\textbf{ALA 2017}} \\ \hline
\multirow{7}*{\textbf{\begin{tabular}[c]{@{}c@{}}ACCURACY\\ for the\\ covariate\\ caste\\ on the\\ test sets\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}RP\end{tabular} & & 0.1 & & 0.11   &   & 0.08
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}MRF\end{tabular} &  & 0.314 $\pm$  0.017  & & 0.316 $\pm$  0.010  &  & 0.556 $\pm$  0.017  
\\ \cline{2-8} 
& MT  & $C = 12$  & ---  & $C = 6$  & ---  & $C = 10$ & ---  
\\ \cline{2-8} 
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.337 $\pm$  0.035         
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & \textbf{0.376 $\pm$  0.023}         
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.598 $\pm$  0.036
\\ \cline{2-8} 
& MTCov  
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & \textbf{0.364 $\pm$  0.048} 
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & 0.371 $\pm$  0.031 
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.625 $\pm$  0.034} 
\\ \hline
\multirow{5}*{\textbf{\begin{tabular}[c]{@{}c@{}}AUC for the\\ link prediction\\ on the\\ test sets\end{tabular}}}     
& MT  & $C = 12$  & \textbf{0.851 $\pm$  0.007} & $C = 6$  & 0.857 $\pm$  0.008  & $C = 10$ & 0.866 $\pm$  0.006          
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.830 $\pm$  0.008          
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & 0.851 $\pm$  0.007 
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.879 $\pm$  0.008
\\ \cline{2-8} 
& MTCov 
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & 0.843 $\pm$  0.005
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & \textbf{0.859 $\pm$  0.005} 
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.889 $\pm$  0.005} 
\\ \hline
\end{tabular}}
\caption{Setting tpe $=0.002$. Performance of methods \textit{MT} , restricted \textit{MTCov}  and \textit{MTCov}  on three social networks and in a sampling bias framework, where the number of edges in the training set is much higher than the number in the test set. RP is the random probability baseline for the accuracy of the category of caste attribute prediction. MRF indicates the maximum relative frequency linked to the covariate caste in the training set. The results are averaged over ten independent runs and the best outcomes are bolded.}
\label{tab: res2}
\end{table}

\begin{table}[htp]
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline  &  & \multicolumn{2}{c}{\textbf{TEN 2013}}  & \multicolumn{2}{c}{\textbf{TEN 2017}} & \multicolumn{2}{c}{\textbf{ALA 2017}} \\ \hline
\multirow{7}*{\textbf{\begin{tabular}[c]{@{}c@{}}ACCURACY\\ for the\\ covariate\\ caste\\ on the\\ test sets\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}RP\end{tabular} & & 0.1 & & 0.11   &   & 0.08
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}MRF\end{tabular} &  & 0.317 $\pm$  0.010  & & 0.317 $\pm$  0.012  &  & 0.566 $\pm$  0.014  
\\ \cline{2-8} 
& MT  & $C = 12$  & ---  & $C = 6$  & ---  & $C = 10$ & ---  
\\ \cline{2-8} 
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.312 $\pm$  0.019         
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & \textbf{0.363 $\pm$  0.036}          
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.564 $\pm$  0.034          
\\ \cline{2-8} 
& MTCov  
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & \textbf{0.326 $\pm$  0.025} 
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & 0.335 $\pm$  0.037
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.613 $\pm$  0.030} 
\\ \hline
\multirow{5}*{\textbf{\begin{tabular}[c]{@{}c@{}}AUC for the\\ link prediction\\ on the\\ test sets\end{tabular}}}     
& MT  & $C = 12$  & 0.711 $\pm$  0.011 & $C = 6$  & 0.741 $\pm$  0.010  & $C = 10$ & 0.752 $\pm$  0.008          
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular}                                                                 
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.698 $\pm$  0.009          
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & 0.745 $\pm$  0.001          
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.777 $\pm$  0.009          
\\ \cline{2-8} 
& MTCov                                                                                                                       
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & \textbf{0.737 $\pm$  0.008}          
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & \textbf{0.766 $\pm$  0.012} 
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.834 $\pm$  0.010} 
\\ \hline
\end{tabular}}
\caption{Setting tpe $=0.01$. Performance of methods \textit{MT} , restricted \textit{MTCov}  and \textit{MTCov}  on three social networks and in a sampling bias framework, where the number of edges in the training set is a bit smaller than the number in the test set. RP is the random probability baseline for the accuracy of the category of caste attribute prediction. MRF indicates the maximum relative frequency linked to the covariate caste in the training set. The results are averaged over ten independent runs and the best outcomes are bolded.}
\label{tab: res3}
\end{table}

\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline  &  & \multicolumn{2}{c}{\textbf{TEN 2013}}  & \multicolumn{2}{c}{\textbf{TEN 2017}} & \multicolumn{2}{c}{\textbf{ALA 2017}} \\ \hline
\multirow{7}*{\textbf{\begin{tabular}[c]{@{}c@{}}ACCURACY\\ for the\\ covariate\\ caste\\ on the\\ test sets\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}RP\end{tabular} & & 0.1 & & 0.11   &   & 0.08
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}MRF\end{tabular} &  & \textbf{0.311 $\pm$  0.012}  & & 0.321 $\pm$  0.017 & & 0.562 $\pm$ 0.017  
\\ \cline{2-8} 
& MT  & $C = 12$  & ---  & $C = 6$  & ---  & $C = 10$ & ---  
\\ \cline{2-8} 
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.303 $\pm$  0.033         
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & \textbf{0.332 $\pm$  0.044}         
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.545 $\pm$  0.032          
\\ \cline{2-8} 
& MTCov  
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & 0.274 $\pm$  0.045 
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & 0.279 $\pm$  0.045 
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.571 $\pm$  0.044} 
\\ \hline
\multirow{5}*{\textbf{\begin{tabular}[c]{@{}c@{}}AUC for the\\ link prediction\\ on the\\ test sets\end{tabular}}}     
& MT  & $C = 12$  & 0.589 $\pm$  0.007 & $C = 6$  & 0.669 $\pm$  0.014  & $C = 10$ & 0.645 $\pm$  0.008          
\\ \cline{2-8}
& \begin{tabular}[c]{@{}c@{}}Restricted \\ MTCov\end{tabular}                                                                 
& \begin{tabular}[c]{@{}c@{}}$C = 12$\\ $\gamma = 0$\end{tabular}   & 0.592 $\pm$  0.017          
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0$\end{tabular}   & 0.656 $\pm$  0.012          
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0$\end{tabular}  & 0.675 $\pm$  0.012          
\\ \cline{2-8} 
& MTCov                                                                                                                      
& \begin{tabular}[c]{@{}c@{}}$C = 10$\\ $\gamma = 0.4$\end{tabular} & \textbf{0.637 $\pm$  0.014}          
& \begin{tabular}[c]{@{}c@{}}$C = 6$\\ $\gamma = 0.5$\end{tabular} & \textbf{0.687 $\pm$  0.016} 
& \begin{tabular}[c]{@{}c@{}}$C = 9$\\ $\gamma = 0.6$\end{tabular} & \textbf{0.759 $\pm$  0.009} 
\\ \hline
\end{tabular}}
\caption{Setting tpe $=0.015$. Performance of methods \textit{MT} , restricted \textit{MTCov}  and \textit{MTCov}  on three social networks and in a sampling bias framework, where the number of edges in the test set is much higher than the number in the training set. RP is the random probability baseline for the accuracy of the category of caste attribute prediction. MRF indicates the maximum relative frequency linked to the covariate caste in the training set. The results are averaged over ten independent runs and the best outcomes are bolded.}
\label{tab: res4}
\end{table}

\noindent Overall, \textit{MTCov}  achieves the highest AUC and the performances of our model in the complex settings are significantly better with respect to the comparison models. This confirms how the presence of another source of information helps in situations that lack positive examples, which in principle would guide the predictions of the test set to the over-represented `population' in the training set. Instead, \textit{MTCov}  performed reasonably well without falling below $63\%$, value well above the baseline of $50\%$ given by the purely random choice. Furthermore, our model achieves better accuracy in the majority of cases, and when \textit{MTCov} is not the best, it is outperformed by its restriction version. Nonetheless, in the single case where our method poorly performs in the caste prediction (Table \ref{tab: res4}), the loss in the accuracy measure is offset by a good performance in the link prediction.


\subsection{Interpretability}
\label{int}

Until now, we presented a quantitative analysis, which lead to prove the robustness of our model and the importance of including the compositional dimensional when detecting communities. Now, we present a qualitative interpretation of the groups detected by \textit{MTCov}  and \textit{MT} . Due to the lack of ground truth and to the presence of overlapping communities, there are not objective rules for analyzing or assigning labels to the communities. 
\begin{figure}[!ht]
\centering
\includegraphics[width=1.0\textwidth]{./Figures/mtcov_ala17.png}
\caption{Partition of the attribute caste inside each community detected by \textit{MTCov}  algorithm in ALA 2017 network.}
\label{fig: com_mtcov}
\end{figure}
However, since the scaling parameter has been estimated between $0.4$ and $0.6$, it highlights a correlation between communities and attribute caste, which can be used as a guide for giving an interpretation of the detected groups. We investigate also if the extra groups detected by \textit{MT} are reallocated by \textit{MTCov}  or if there is an overall topological change between the two methods. Figures \ref{fig: com_mtcov} and \ref{fig: com_mt} refer to the network ALA 2017, while the plots for the `Te\underline{n}pa\d{t}\d{t}i' networks are attached in Appendix \ref{AB}. They show the partition of the attribute caste inside each community, detected by \textit{MTCov}  and \textit{MT} respectively. They display a notable difference in the composition of the groups with respect to the covariate: while \textit{MT} keeps the same proportions of the categories inside each group, \textit{MTCov}  discriminates better, especially between the most representative categories, that have the maximum relative frequency in at least one community. 
\begin{figure}[!ht]
\centering
\includegraphics[width=1.0\textwidth]{./Figures/mt_ala17.png}
\caption{Partition of the attribute caste inside each community detected by \textit{MT} algorithm in ALA 2017 network.}\label{fig: com_mt}
\end{figure}

\begin{table}[ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
                         & \multicolumn{2}{c}{\textbf{TEN 2013}}          & \multicolumn{2}{c}{\textbf{TEN 2017}}        & \multicolumn{2}{c}{\textbf{ALA 2017}}         \\ \hline
                         & \textbf{\begin{tabular}[c]{@{}c@{}}\textit{MT} \\ ($C=12$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MTCov \\ ($C=10$)\end{tabular}} & 
                         \textbf{\begin{tabular}[c]{@{}c@{}}MT \\ ($C=6$)\end{tabular}} & 
                         \textbf{\begin{tabular}[c]{@{}c@{}}MTCov \\ ($C=6$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MT \\ ($C=10$)\end{tabular}} & 
                         \textbf{\begin{tabular}[c]{@{}c@{}}MTCov \\ ($C=9$)\end{tabular}} \\ \hline
\textbf{Aasaari}         & 12                   & 9                       & 6                   & 5                      & 6                    & 2                      \\
\textbf{Agamudaiyaan}    & 12                   & 10                      & 6                   & 6                      & -                  & -                    \\
\textbf{Arundhathiyar}   & 7                    & 7                       & 6                   & 5                      & 9                    & 6                      \\
\textbf{Hindu Vellalar}  & 1                    & 3                       & 3                   & 1                      & 5                    & 1                      \\
\textbf{Hindu Yaathavar} & 12                   & 10                      & 6                   & 6                      & 10                   & 8                      \\
\textbf{Ilavaa}          & -                  & -                     & -                 & -                    & 4                    & 2                      \\
\textbf{Jaanaan}         & -                  & -                     & -                 & -                    & 5                    & 2                      \\
\textbf{Kallar}          & 11                   & 9                       & 5                   & 2                      & -                  & -                    \\
\textbf{Kulaalar}        & 9                    & 2                       & 6                   & 3                      & 10                   & 6                      \\
\textbf{Maravar}         & -                  & -                     & -                 & -                    & 10                   & 9                      \\
\textbf{Naayakkar}       & 5                    & 3                       & -                 & -                    & -                  & -                    \\
\textbf{Pallar}          & 12                   & 10                      & 6                   & 6                      & 10                   & 9                      \\
\textbf{Pandaaram}       & -                  & -                     & -                 & -                    & 5                    & 5                      \\
\textbf{Paraiyar}        & -                  & -                     & -                 & -                    & 10                   & 8                      \\
\textbf{Pillamaar}       & -                  & -                     & -                 & -                    & 3                    & 2                      \\
\textbf{RC Vellalar}     & -                  & -                     & -                 & -                    & 8                    & 5                      \\
\textbf{RC Yaathavar}    & 12                   & 10                      & 6                   & 6                      & -                  & -                    \\ \hline
\end{tabular}%
}
\caption{Number of communities in which each category is present, for each network and method.}
\label{tab: numbers_com}
\end{table}

\noindent This is also confirmed by the number of communities in which each category is present, shown in Table \ref{tab: numbers_com}. Although \textit{MTCov}  favors a smaller number of communities than \textit{MT}, the differences between the two models are considerable. A clear example is given by the network TEN 2017, where a fair comparison is possible due to the same estimate of the hyperparameter $C$. In this framework, \textit{MTCov}  never allocates the categories in a greater number of communities than \textit{MT}, and it keeps each of them in as few communities as possible.
For this reason, the groups detected by our model seem to respect both influence of the network topology and the node attribute, creating communities that are not only structurally close but also share common characteristics. On the other hand, instead, the compositional structure of the \textit{MT} communities is quite random and doesn't show any correlation between the communities and the covariate. However, this is at the expense of the size of the groups, which in the \textit{MTCov}  case are unbalanced. One might argue that, given that \textit{MTCov}  incorporates the covariate in the model, it should be expected to observe a correlation with the inferred communities. However, the estimate for the hyperparameter $\gamma$ has been done in a range which involved also 0 (the closest situation to the \textit{MT} case), but in all three cases the final estimate is different from the null value, underlying an interdependence between covariate, communities and structure. On the other hand, since we have never estimated $\gamma=1$, we did not expect that the communities would fit completely the caste resulting in a clustering problem. A more complete and explanatory representation can be found in Figure \ref{fig: representation}. 
\begin{figure}[!ht]

\centering

\bigskip
\begin{minipage}[b]{\textwidth}
\centering
\subfloat{\includegraphics[width=.37\linewidth]{./Figures/ten17_caste.png}}
\caption*{(a) Caste partition.}
\end{minipage}

\bigskip
\begin{minipage}[b]{\textwidth}
\centering
\subfloat{\includegraphics[width=.33\linewidth]{./Figures/ten17_1.png}}
\subfloat{\includegraphics[width=.33\linewidth]{./Figures/ten17_2.png}}
\subfloat{\includegraphics[width=.33\linewidth]{./Figures/ten17_3.png}}
\caption*{(b) Community 1, Community 2, Community 3.}
\end{minipage}

\bigskip
\begin{minipage}[b]{\textwidth}
\centering
\subfloat{\includegraphics[width=.33\linewidth]{./Figures/ten17_4.png}}
\subfloat{\includegraphics[width=.33\linewidth]{./Figures/ten17_5.png}}
\subfloat{\includegraphics[width=.33\linewidth]{./Figures/ten17_6.png}}
\caption*{(c) Community 4, Community 5, Community 6.}
\end{minipage}

\caption{TEN 2017 community partition. On top, the division by caste membership. Subplots (b) and (c) show the membership in each of the 6 communities for each node, with color ranging from white
if the out-going membership $u_{ik} = 0$ to black if $u_{ik} = 1$. Values in between denote overlapping membership (grey).}
\label{fig: representation}
\end{figure}
It represents the TEN 2017 network with the grouped links of the layers, together with its predicted community assignment and the division of individuals into castes (image (a)). Subplots (b) and (c) display the membership in each of the 6 communities for each node, with a grey scale color. The black corresponds to values $1$ in the membership matrix $\hat{U}$, while the white is linked with $0$. The greys denote the overlapping membership.
Overall, the predicted communities show a relationship with the caste partition, more evident in communities 2 and 4, and weak in community 1. Notice also the different sizes of the groups. Finally, these results suggest that there may be other attributes related to the communities.



==> preamble/preamble_acronyms.tex <==
\hyphenation{cdebacco}
\newcommand{\CDB}[1]{\textcolor{red}{#1}}
\newcommand{\CDBcom}[1]{[\textcolor{red}{CDB: #1}]}
\newcommand{\dave}[1]{\textcolor{blue}{#1}}
\newcommand{\davecom}[1]{[\textcolor{blue}{DL: #1}]}
\newcommand{\EB}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\EBcom}[1]{[\textcolor{ForestGreen}{CM: #1}]}
\newcommand{\nix}[1]{\textcolor{lightgray}{#1}}
